DyPS: Dynamic Processor Switching for Energy-Aware Video Decoding on Multi-core SoCs

In addition to General Purpose Processors (GPP), Multicore SoCs equipping modern mobile devices contain specialized Digital Signal Processor designed with the aim to provide better performance and low energy consumption properties. However, the experimental measurements we have achieved revealed that system overhead, in case of DSP video decoding, causes drastic performances drop and energy efficiency as compared to the GPP decoding. This paper describes DyPS, a new approach for energy-aware processor switching (GPP or DSP) according to the video quality . We show the pertinence of our solution in the context of adaptive video decoding and describe an implementation on an embedded Linux operating system with the help of the GStreamer framework. A simple case study showed that DyPS achieves 30% energy saving while sustaining the decoding performance

==> code.tex <==
The \textit{handler.c} source code listed below shows how the processor switching mechanism is achieved.  In Line 1 and 2, ARM and DSP decoder are instantiated. At line 44, start the "New Pad" handler where the decoder selection is done at line 10 according to the new video content resolution. The dynamic pluging is done in line  13, 17 and 19.   
\noindent 
\lstset{
  language=C,                % choose the language of the code
  numbers=left,                   % where to put the line-numbers
  stepnumber=1,                   % the step between two line-numbers.        
  numbersep=5pt,                  % how far the line-numbers are from the code
  backgroundcolor=\color{mygray},  % choose the background color. You must add \usepackage{color}
  showspaces=false,               % show spaces adding particular underscores
  showstringspaces=false,         % underline spaces within strings
  showtabs=false,                 % show tabs within strings adding particular underscores
  tabsize=2,                      % sets default tabsize to 2 spaces
  captionpos=b,                   % sets the caption-position to bottom
  breaklines=true,                % sets automatic line breaking
  breakatwhitespace=true,         % sets if automatic breaks should only happen at whitespace
  title=handler.c,                 % show the filename of files included with \lstinputlisting;
}
\lstinputlisting{sources/handler.c}


\subsection{Requirements}
In the proposed solution,  the switching between the execution processors should : 

\begin{enumerate}

\item  occurs dynamically
\item be done seamlessly.
\item have low overhead.

\end{enumerate}

The objective of these requirement is to allow the processor switching to occur dynamically as reaction to a dynamic adaptation in the video quality. This should be achieved seamlessly to the user application a have a low overhead so to not  impact the video playback quality.

